Event-triggered Learning for Resource-efficient Networked Control

Common event-triggered state estimation (ETSE) algorithms save communication in networked control systems by predicting agents' behavior, and transmitting updates only when the predictions deviate significantly. The effectiveness in reducing communication thus heavily depends on the quality of the dynamics models used to predict the agents' states or measurements. Event-triggered learning is proposed herein as a novel concept to further reduce communication: whenever poor communication performance is detected, an identification experiment is triggered and an improved prediction model learned from data. Effective learning triggers are obtained by comparing the actual communication rate with the one that is expected based on the current model. By analyzing statistical properties of the inter-communication times and leveraging powerful convergence results, the proposed trigger is proven to limit learning experiments to the necessary instants. Numerical and physical experiments demonstrate that event-triggered learning improves robustness toward changing environments and yields lower communication rates than common ETSE.

==> texs/9bib.tex <==
\begin{thebibliography}{99}

\bibitem{c1} Trimpe, Sebastian. "Event-based state estimation with switching static-gain observers." IFAC Proceedings Volumes 45.26 (2012): 91-96.
\bibitem{c2} Hespanha, J. P., and Y. Xu. "Communication logics for networked control systems." Proceedings of the 2004 American Control Conference. 2004.
\bibitem{c3} Schuss, Zeev. Theory and applications of stochastic processes: an analytical approach. Vol. 170. Springer Science \& Business Media, 2009.
\bibitem{c4} Kifer, Daniel, Shai Ben-David, and Johannes Gehrke. "Detecting change in data streams." Proceedings of the Thirtieth international conference on Very large data bases-Volume 30. VLDB Endowment, 2004.
\bibitem{c5}
\bibitem{c6}
\bibitem{c7} 
\bibitem{c8} 
\bibitem{c9} 

\end{thebibliography}

